Mirror Descent Maximizes Generalized Margin and Can Be Implemented Efficiently

Driven by the empirical success and wide use of deep neural networks, understanding the generalization performance of overparameterized models has become an increasingly popular question. To this end, there has been substantial effort to characterize the implicit bias of the optimization algorithms used, such as gradient descent (GD), and the structural properties of their preferred solutions. This paper answers an open question in this literature: For the classification setting, what solution does mirror descent (MD) converge to? Specifically, motivated by its efficient implementation, we consider the family of mirror descent algorithms with potential function chosen as the $p$-th power of the $\ell_p$-norm, which is an important generalization of GD. We call this algorithm $p$-$\textsf{GD}$. For this family, we characterize the solutions it obtains and show that it converges in direction to a generalized maximum-margin solution with respect to the $\ell_p$-norm for linearly separable classification. While the MD update rule is in general expensive to compute and perhaps not suitable for deep learning, $p$-$\textsf{GD}$ is fully parallelizable in the same manner as SGD and can be used to train deep neural networks with virtually no additional computational overhead. Using comprehensive experiments with both linear and deep neural network models, we demonstrate that $p$-$\textsf{GD}$ can noticeably affect the structure and the generalization performance of the learned models.

==> introduction_old.tex <==



\section{Introduction}
\begin{comment}
Outline:
\begin{enumerate}
    \item Overparameterization
    \item prior results on the bias of GD
    \item MD as the generalization of GD
    \item SMD w/ $p$-norm is practical
    \item regression vs/ classification (knowledge gap)
    \item bias of SMD in classification
    \item experiments -- $\ell_\infty$ has the best generalization
\end{enumerate}
\end{comment}

Deep and overparameterized models have enjoyed tremendous amount of success in a wide range of machine learning applications~\citep{krizhevsky2012imagenet, lecun2015deep, mnih2015human, silver2016mastering}.
But, as these highly expressive models have the capacity to have multiple solutions that interpolate training data, it is important to characterize which of these interpolating solutions  optimization algorithms converge to.
Such characterization is especially important as it will help us understand the generalization performance of the models, one of the most important questions in machine learning.
Traditionally, people had incorporated explicit penalties on the model complexities, such as ridge regularization, to induce solutions that avoid overfitting.
Recent research highlighted that many optimization methods implicitly regularize the learned models without being specified in the learning objectives, and such inherently bias plays a crucial role in the generalization performance of deep learning~\citep{neyshabur2014search, zhang2021understanding, wilson2017marginal}.
Therefore, we must realize that the models only tell half of the story about the generalization performance of learning -- the optimization algorithm used to train these models also play a key role.

It had been shown that various optimization algorithms can exhibit biases towards different implicit regularization.
For example, it has been shown that for logistics loss, gradient descent iterates converge to the $\ell_2$-maximum margin SVM solution~\citep{soudry2018implicit}.
And \cite{wilson2017marginal} showed that various adaptive variants of SGD have different implicit regularization.
Analysis for other optimization methods, including AdaBoost and steepest descent had also appeared in recent literature~\citep{telgarsky2013margins,gunasekar2018characterizing,rosset2004boosting}.
Notably, implicit regularization can depend on the loss function, e.g. the steepest descent algorithm implicitly regularizes for exponential loss but not for quadratic loss.

In this paper, we will advance the understanding of the implicit regularization of the mirror descent algorithm, which is a generalization of the popular gradient descent algorithm.
The mirror descent algorithm uses a convex potential function $\psi$ generalize the Euclidean geometry and its iterative updates can be defined as $\nabla\psi(w_{t+1}) = \nabla\psi(w_t) - \eta L(w_t)$.
In the case where $\psi = \frac{1}{2} \norm{\cdot}_2^2$, this is equivalent to gradient descent.
Another popular example of mirror descent is when $\psi$ is taken to be the negative entropy, and this case is equivalent to the hedge algorithm.
The implicit regularization of mirror descent had been studied in the past, \citep{gunasekar2018characterizing, azizan2018stochastic} had shown that for regression problems, mirror descent converges to the interpolating solution that is closest to the initialization (with respect to the distance generated by $\psi$).
And in this paper, we will extend our understanding to the setting of classification problems.


We believe that mirror descent is interesting because it can efficiently implemented in practice.
Although many optimization algorithms for machine learning had been proposed over the years, in practice people predominantly only utilize gradient descent and its adaptive variants.
One reason is that gradient descent updates can be applied coordinate-wise, in the sense that outside of computing the loss, updating the value at one coordinate does not depend on the values at other coordinate.
This \textit{separability} property of gradient descent allows it to be easily parallelized and better take advantage of modern computing hardware such as GPUs.
In this paper, we make the important observation that, under appropriate choice of the mirror map, mirror descent is separable just like gradient descent.
Therefore, we apply mirror descent to take advantage of its implicit regularization, while nearly matching gradient descent in computational performance.

\paragraph{Our Contributions.}
In this paper, we offer the following contributions in both the theoretical and empirical aspects of the study of implicit regularization:

\begin{table}[b]
\centering
\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{10pt}
\begin{tabular}{ |c |c|c| }
\hline  & Regression & Classification  \\
\hline\hline  
\multirow{3}{*}{\begin{tabular}{c}Gradient Descent\\($\mir(\cdot) = \frac{1}{2}\norm{\cdot}_2^2$)\end{tabular}}  & $\argmin_w \norm{w-w_0}_2$ & $\argmin_w \norm{w}_2$  \\
 & $\st~~w \text{ fits all data} $ & $\st~~w \text{ classifies all data} $    \\
 & 
\citep[Thm 6.1]{engl1996regularization} & \cite{soudry2018implicit}   \\
   \hline \hline
 \multirow{4}{*}{\begin{tabular}{c}Mirror Descent\\($\mir(\cdot) = \frac{1}{p}\norm{\cdot}_p^p$)\end{tabular}}  & $\argmin_w \norm{w-w_0}_p$ & $\argmin_w \norm{w}_p$  \\
 & $\st~~w \text{ fits all data} $ & $\st~~w \text{ classifies all data} $    \\
 & 
\cite{gunasekar2018characterizing} & \high{This work}  \\
& \cite{azizan2018stochastic} & \\
  \hline 
\end{tabular}
\label{tab:sto1} 
\caption{{\bf Conceptual summary of our results.}\tba{add caption \& make the contents more rigorous / precise} 
 }
\end{table}
\begin{list}{{\tiny $\blacksquare$}}{\leftmargin=1.5em}
  \setlength{\itemsep}{-1pt}
    \item We propose that mirror descent with potential $\frac{1}{p}\norm{\cdot}_p^p$, which will call \algname, is a practical and efficient alternative to gradient descent.
    \item We show that for linear models and any loss satisfying Assumption~\ref{assum:class-loss}, \algname exhibits implicit regularization by following the so-called regularization path, which we will formally define in Section~\ref{sec:priliminaries}.
    And for logistics loss, this is equivalent to convergence to the maximum hard-margin SVM solution with respect to the $\ell_p$ norm.
    \item We illustrate the power of having a different implicit regularization using a set of extensive experiments with deep neural network models and the CIFAR-10~\citep{krizhevsky2009learning} and Imagenet~\citep{russakovsky2015imagenet} datasets.
    These results show that our theoretical result in fact translate into the highly nonlinear setting very well.
    Most importantly, we show that a choice of larger $p$ generalizes much better than gradient descent (which is equivalent to when $p=2$), regardless of the underlying neural network architecture.
\end{list}

We hope this paper both closes a gap in the theoretical understanding of implicit regularization, and presents a practical and efficient approach to apply such knowledge in improving the performance of machine learning models.

%\tba{add a table with the missing part}
